Contrast then Memorize: Semantic Neighbor Retrieval-Enhanced Inductive Multimodal Knowledge Graph Completion

A large number of studies have emerged for Multimodal Knowledge Graph Completion (MKGC) to predict the missing links in MKGs. However, fewer studies have been proposed to study the inductive MKGC (IMKGC) involving emerging entities unseen during training. Existing inductive approaches focus on learning textual entity representations, which neglect rich semantic information in visual modality. Moreover, they focus on aggregating structural neighbors from existing KGs, which of emerging entities are usually limited. However, the semantic neighbors are decoupled from the topology linkage and usually imply the true target entity. In this paper, we propose the IMKGC task and a semantic neighbor retrieval-enhanced IMKGC framework CMR, where the contrast brings the helpful semantic neighbors close, and then the memorize supports semantic neighbor retrieval to enhance inference. Specifically, we first propose a unified cross-modal contrastive learning to simultaneously capture the textual-visual and textual-textual correlations of query-entity pairs in a unified representation space. The contrastive learning increases the similarity of positive query-entity pairs, therefore making the representations of helpful semantic neighbors close. Then, we explicitly memorize the knowledge representations to support the semantic neighbor retrieval. At test time, we retrieve the nearest semantic neighbors and interpolate them to the query-entity similarity distribution to augment the final prediction. Extensive experiments validate the effectiveness of CMR on three inductive MKGC datasets. Codes are available at https://github.com/OreOZhao/CMR.

==> figs/intro_knn.tex <==
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.49\textwidth]{figs/intro_knn2.pdf}
    \caption{Semantic neighbors of query (\textit{WALL-E}, \textit{production companies}) involving the emerging entity \textit{WALL-E}. Existing IKGC methods utilize structural neighbors (Figure \ref{fig:intro_knn} left) while we propose to aggregate the semantic neighbors (Figure \ref{fig:intro_knn} right). }
    \label{fig:intro_knn}
\end{figure}

% \begin{figure}[t]
% \centering
% \subfigure[]{
% \label{fig:intro_knn}
% \includegraphics[width=0.48\textwidth]{figs/intro_knn2.pdf}}
% \subfigure[Multimodal semantic correlation (shading of texts and image) between query (\textit{WALL-E}, \textit{production companies}) and its target \textit{Pixar}.]{
% \label{fig:intro_clip}
% \includegraphics[width=0.48\textwidth]{figs/intro_clip4.pdf}}
% \caption{
% Moreover, we propose to capture both textual-textual and textual-visual correlation in the query-entity pair (Figure \ref{fig:intro_clip}).}
% \end{figure}

==> tables/vis.tex <==
\begin{table}[t!]
\caption{The token-wise similarity between query \textit{(Jeff Garlin, perform)} and ground-truth entity \textit{WALL-E (e1))}, and irrelevant entity \textit{Public University (e2)}.
}
\small
\centering
\resizebox{0.49\textwidth}{!}{
\begin{tabular}[t]{p{4cm}p{4cm}}
\toprule
\textbf{\textit{WALL-E } \textcolor{blue}{\cmark}}     & \textbf{\textit{Public University } \textcolor{red}{\xmark}}
\\
\midrule
\multicolumn{2}{l}{\textbf{\textit{Visualization of Attention Weights}}} \\
\multicolumn{2}{c}{
% \raisebox{-0.95\totalheight}{
    \includegraphics[width=1.1\linewidth]{figs/e2attn.pdf} 
% }
}
\\
\midrule
\multicolumn{2}{l}{\textbf{\textit{Rankings of Entity Candidates}}} \\
\entity{Thailand}, Malaysia, Hong Kong, Khmer language, Khuang Aphaiwong, Cambodia, Patna, \entity{Singapore}, ...
& 
\entity{Singapore}, Indonesian language, Javanese language, West Sumatra, Malaysia, \entity{Thailand}, Jakarta Cambodia, Patna, ... \\
\bottomrule
\end{tabular}
}
\label{tab: case}
\end{table}
